Minimizing the Size of the Uncertainty Regions for Centers of Moving Entities

In this paper, we study the problems of computing the 1-center, centroid, and 1-median of objects moving with bounded speed in Euclidean space. We can acquire the exact location of only a constant number of objects (usually one) per unit time, but for every other object, its set of potential locations, called the object's uncertainty region, grows subject only to the speed limit. As a result, the center of the objects may be at several possible locations, called the center's uncertainty region. For each of these center problems, we design query strategies to minimize the size of the center's uncertainty region and compare its performance to an optimal query strategy that knows the trajectories of the objects, but must still query to reduce their uncertainty. For the static case of the 1-center problem in R^1, we show an algorithm that queries four objects per unit time and is 1-competitive against the optimal algorithm with one query per unit time. For the general case of the 1-center problem in R^1, the centroid problem in R^d, and the 1-median problem in R^1, we prove that the Round-robin scheduling algorithm is the best possible competitive algorithm. For the center of mass problem in R^d, we provide an O(log n)-competitive algorithm. In addition, for the general case of the 1-center problem in R^d (d >= 2), we argue that no algorithm can guarantee a bounded competitive ratio against the optimal algorithm.

==> 1_median_orig.tex <==
\section{The 1-Median Problem}
\label{ch:1median}

%In this section, we study the $1$-median problem with moving entities. For this problem in $\mathbb{R}^1$, we prove that the Round-robin algorithm keeps the maximum size of the uncertainty region within $O(v  n)$ and achieves the best possible competitive ratio of $O(n)$ against the optimal algorithm. In addition, we argue that for the optimal algorithm, the maximum size of the uncertainty region can be $\Omega(v  n)$. For the case where objects have different maximum speeds, we show that the Round-robin algorithm achieves a competitive ratio of $O(v_M  n / v_m)$, where $v_M$ is the highest maximum speed and $v_m$ is the lowest maximum speed. Finally, for the $1$-median problem in $\mathbb{R}^d$ ($d \geq 2$), we show that the maximum size of the uncertainty region can be unbounded for the optimal algorithm.

Given a set of $n$ points in $\mathbb{R}^1$, for $1 \leq k \leq n$, we define the $k$-th smallest problem as finding the position of the $k$-th smallest point. %Hence, when $n$ is odd, the $1$-median problem is the same as the $\lceil \frac{n}{2} \rceil$-th smallest problem. Moreover, when $n$ is even, we consider the $1$-median to be the midpoint of the $\frac{n}{2}$-th smallest and $(\frac{n}{2}+1)$-th smallest points. In this case, the size of the uncertainty region for the $1$-median is equivalent to the average of the size of the uncertainty region for the $\frac{n}{2}$-th smallest and the size of the uncertainty region for the $(\frac{n}{2}+1)$-th smallest.
We introduce a lemma regarding the $k$-th smallest problem which we will later use to prove Theorem~\ref{thm:1medmain}.
The proof of the lemma is provided in Appendix~\ref{app:klow}.

\begin{lemma} \label{lem:klow}
%When $n \geq 3$, for the $k$-th smallest problem ($2 \leq k \leq n-1$), the maximum size of the uncertainty region over all time is $\Omega(v)$, regardless of the query strategy.
 The maximum size of the uncertainty region of the $k$-th smallest ($2 \leq k \leq n-1$), over all time is $\Omega(v)$, regardless of the query strategy.
\end{lemma}

\begin{comment}
\begin{proof}
We prove this by contradiction.
We assume that there exists an example where using an algorithm $A$, the size of the uncertainty region for the $k$-th smallest problem will never exceed $\frac{v}{2}$.
For $1 \leq i \leq n$ and $q \geq 0$, let $s_{i, q}$ ($e_{i, q}$) be equal to the $i$-th smallest starting (ending) point among the starting (ending) points of the uncertainty regions of all objects after exactly $q$ queries are made by $A$.
We say that $s_{i, q}$ ($e_{i, q}$) bounds an object $b$ if it is equal to the starting (ending) point of the uncertainty region of $b$.
$[s_{i, q}, e_{i, q}]$ is the uncertainty region for the $i$-th smallest problem after $q$ queries. 
By our assumption, $e_{k, q}-s_{k, q} \leq \frac{v}{2}$ for all $q$.
%\will{for all $q$ (and consider using $q$ instead of $j$)}.

%Therefore, at most one uncertainty region with a starting point greater than or equal to $s_{k,q}$ can have an ending point less than or equal to $e_{k,q}$ and the object with that uncertainty region must have been queried last. Hence, all $k-1$ uncertainty regions with a starting point less than or equal to $s_{k-1,q}$ must have an ending point less than or equal to $e_{k,q}$. Consequently, the uncertainty region of no object starts before $s_{k,q}$ and ends after $e_{k,q}$.

Let us consider the case that for some $q \geq 0$, we have $e_{k, q} - e_{k-1, q} \leq \frac{v}{2}$. If $s_{k+1, q} \leq e_{k, q}$, after the $(q+1)$-th query, we will have at least $k$ starting points less than or equal to $e_{k, q} - v$. Also, we will have $e_{k, q+1} \geq e_{k-1, q} + v$. Thus, we will have $s_{k, q+1} \leq e_{k, q} - v \leq e_{k-1, q} - \frac{v}{2} \leq e_{k, q+1} - \frac{3v}{2}$. However, this is against the assumption that using algorithm $A$, the size of the uncertainty region for the $k$-th smallest problem will never exceed $\frac{v}{2}$. Consequently, we must have $s_{k+1, q} > e_{k, q}$. If the $(q+1)$-th query acquires the exact location of the object that was bounded by $e_{k, q}$ after $q$ queries, the new position of that object must be greater than or equal to $e_{k-1, q} + \frac{v}{2}$ so that we have $e_{k, q+1}-s_{k, q+1} \leq \frac{v}{2}$. In that case, we have $e_{k, q+1} \geq e_{k, q} + \frac{v}{2}$ and $e_{k, q+1} - e_{k-1, q+1} \leq \frac{v}{2}$. If the $(q+1)$-th query acquires the exact location of any other object, the starting point of the uncertainty region of that object before the $(q+1)$-th query must have been less than or equal to $s_{k, q}$ (this is a necessary condition for having $e_{k, q+1}-s_{k, q+1} \leq \frac{v}{2}$). Hence, in that case, $e_{k, q+1} = e_{k, q} + v$. Moreover, the new position of the queried object must be greater than or equal to $e_{k, q} + \frac{v}{2}$ so that we have $e_{k, q+1}-s_{k, q+1} \leq \frac{v}{2}$. For this reason, we have $e_{k, q+1} - e_{k-1, q+1} \leq \frac{v}{2}$. Therefore, in both cases, we have $e_{k, q+1} - e_{k-1, q+1} \leq \frac{v}{2}$, $e_{k, q+1} \geq e_{k, q} + \frac{v}{2}$ and $s_{k+1, q+1} < s_{k+1, q}$. We deduce that for some $q' > q$, we will have $e_{k, q'} - e_{k-1, q'} \leq \frac{v}{2}$ and $s_{k+1, q'} \leq e_{k, q'}$. As a result, the size of the uncertainty region for the $k$-th smallest problem will exceed $\frac{v}{2}$. Hence, if we have $e_{k, q} - e_{k-1, q} \leq \frac{v}{2}$ for some $q \geq 0$, the size of the uncertainty region for the $k$-th smallest problem will exceed $\frac{v}{2}$ which is against the assumption about algorithm $A$. Similarly, we can show that if we have $s_{k+1, q} - s_{k, q} \leq \frac{v}{2}$ for some $q \geq 0$, the size of the uncertainty region for the $k$-th smallest problem will exceed $\frac{v}{2}$ at some point.

We now consider the case that for some $q \geq 0$, $s_{k, q}$ and $e_{k, q}$ bound two different objects. If the object bounded by $e_{k, q}$ was not queried last, then at most $k-2$ ending points can be smaller than $s_{k, q}$; thereby, $s_{k, q} \leq e_{k-1, q}$. Therefore, we have $e_{k, q} - e_{k-1, q} \leq e_{k, q} - s_{k, q} \leq \frac{v}{2}$. If the object bounded by $e_{k, q}$ was queried last, then we have a starting point at $e_{k, q}$. In that case, we have $s_{k+1, q} - s_{k, q} \leq e_{k, q} - s_{k, q} \leq \frac{v}{2}$. We deduce that either $e_{k, q} - e_{k-1, q} \leq \frac{v}{2}$ or $s_{k+1, q} - s_{k, q} \leq \frac{v}{2}$. As a result, the size of the uncertainty region for the $k$-th smallest problem will exceed $\frac{v}{2}$ at some point which is against the assumption about algorithm $A$.

Hence, for every $q \geq 0$, $s_{k, q}$ and $e_{k, q}$ must bound the same object. Furthermore, we must have $e_{k, q} - e_{k-1, q} > \frac{v}{2}$ and $s_{k+1, q} - s_{k, q} > \frac{v}{2}$. Since we assume that $e_{k, q}-s_{k, q} \leq \frac{v}{2}$, we must have the exact location of the object bounded by $s_{k, q}$ and $e_{k, q}$ after $q$ queries. This means that $e_{k, q}-s_{k, q} = 0$ and if $q > 0$, the $q$-th query must have acquired the exact location of the object bounded by $s_{k, q}$ and $e_{k, q}$. If after $q$ queries ($q \geq 0$), we have the exact location of an object $t$, we know that $t$ has the $k$-th smallest position, and we also have $e_{k, q} - e_{k-1, q} > \frac{v}{2}$ and $s_{k+1, q} - s_{k, q} > \frac{v}{2}$, $t$ can potentially have the $k$-th smallest position after the $(q+1)$-th query, regardless of which object will be queried. Thus, no other object $t'$ exists such that we have its exact location after $q+1$ queries and that we know with certainty that it has the $k$-th smallest position. Therefore, if at any point, algorithm $A$ queries an object whose initial position was not the $k$-th smallest, the size of the uncertainty region for the $k$-th smallest problem will eventually exceed $\frac{v}{2}$. On the other hand, if algorithm $A$ always queries the same object $t$ whose initial position was the $k$-th smallest, then the uncertainty regions of the other objects will become extensive. In that case, considering that the initial position of $t$ was the $k$-th smallest ($2 \leq k \leq n-1$), the uncertainty region of at least one other object will include the position of $t$ at some point in the future. When this happens, the position of $t$ will not necessarily be the $k$-th smallest. Consequently, the size of the uncertainty region for the $k$-th smallest problem will exceed $\frac{v}{2}$ at some point.

In every case, we have proved that using algorithm $A$, the size of the uncertainty region for the $k$-th smallest problem will exceed $\frac{v}{2}$. This contradicts our assumption about algorithm $A$. Therefore, for every algorithm, the maximum size of the uncertainty region for the $k$-th smallest problem is greater than $\frac{v}{2}$. Thus, when $2 \leq k \leq n-1$, regardless of the query strategy, the maximum size of the uncertainty region for the $k$-th smallest problem is $\Omega(v)$.

\end{proof}
\end{comment}

We now present the main theorem in this section.
For the $1$-median problem in $\mathbb{R}^1$, we prove that the Round-robin algorithm achieves the best possible competitive ratio against the optimal algorithm.
The proof is provided in Appendix~\ref{app:1medmain}.

\begin{theorem} \label{thm:1medmain}
For the $1$-median problem in $\mathbb{R}^1$, the Round-robin scheduling algorithm keeps the maximum size of the uncertainty region within $O(v  n)$ at any point in the future and achieves the best possible competitive ratio of $O(n)$ against the optimal algorithm.
\end{theorem}

\begin{comment}
\begin{proof}
The Round-robin algorithm keeps the size of the uncertainty region of each object within $O(v  n)$ because it acquires the exact location of each object once in every $n$ queries.
For $1 \leq k \leq n$, let $s_k$ be equal to the $k$-th smallest starting point among the starting points of the uncertainty regions of all objects.
Also, let $e_k$ be equal to the $k$-th smallest ending point among the ending points of the uncertainty regions of all objects.
Hence, $[s_k, e_k]$ is the uncertainty region for the $k$-th smallest.
Using the Round-robin algorithm, we know that $e_k - s_k$ will always be $O(v  n)$ because the algorithm keeps the size of the uncertainty region of each object within $O(v  n)$.
Thus, the size of the uncertainty region for the $k$-th smallest is bounded by $O(v  n)$ at any point in the future.
Therefore, using the Round-robin algorithm, the size of the uncertainty region for the $1$-median will never exceed $O(v  n)$.

If $n=2$, at any point after the first query, the size of the uncertainty region of one of the objects will be $\Omega(v)$. Thus, the maximum size of the uncertainty region for the $1$-median will be $\Omega(v)$.
If $n \geq 3$, by Lemma~\ref{lem:klow}, the maximum size of the uncertainty region for the $k$-th smallest ($2 \leq k \leq n-1$) will be $\Omega(v)$, regardless of the query strategy. 
Therefore, for the optimal algorithm, the size of the uncertainty region for the $1$-median will be $\Omega(v)$ at some point in the future. Considering that the Round-robin algorithm keeps the maximum size of the uncertainty region within $O(v  n)$, it achieves a competitive ratio of $O(n)$ against the optimal algorithm.

%If $n \geq 3$, we argue that for any $2 \leq k \leq n-1$, regardless of the query strategy, the size of the uncertainty region for the $k$-th smallest problem will be $\Omega(v)$ at some point in the future. 

Now, we show that $O(n)$ is the best possible competitive ratio against the optimal algorithm. We consider the following cases:
\begin{itemize}
    \item If $n$ is odd, we consider an example with $\lceil \frac{n}{2} \rceil$ objects initially located at the origin and $\lfloor \frac{n}{2} \rfloor$ objects initially located at $10  v  n$. One of the objects initially located at the origin moves with a speed of $v$ towards $3  v  n$ and then stays there. The rest of the objects do not move. Let us consider an algorithm that acquires the exact location of the moving object once in every two queries (even after the object stops at $3  v  n$) and assigns the rest of the queries to the static objects in a circular order. This algorithm maintains the size of the uncertainty region for the $\lceil \frac{n}{2} \rceil$-th smallest within $O(v)$.
    \item If $n$ is even, we consider an example with $\frac{n}{2}$ objects initially located at the origin and $\frac{n}{2}$ objects initially located at $10  v  n$. One of the objects initially located at the origin moves with a speed of $v$ towards $3  v  n$ and then stays there. Also, one of the objects initially located at $10  v  n$ moves with a speed of $v$ towards $7  v  n$ and then stays there. The rest of the objects do not move. We consider an algorithm that acquires the exact location of each of the two moving objects once in every three queries (even after the objects stop moving) and assigns the rest of the queries to the static objects in a circular order. This algorithm maintains the size of the uncertainty region for the $\frac{n}{2}$-th and $(\frac{n}{2}+1)$-th smallest within $O(v)$.
\end{itemize}
Therefore, in the examples provided for both cases, the optimal algorithm keeps the maximum size of the uncertainty region for the $1$-median within $O(v)$. However, there is no guarantee for any algorithm that does not know the trajectories of the objects, such as Round-robin, to query any moving object in the first $\lceil \frac{n}{2} \rceil - 1$ attempts; hence, the size of the uncertainty region for the $\lceil \frac{n}{2} \rceil$-th smallest can become $\Omega(v  n)$ after the first $\lceil \frac{n}{2} \rceil - 1$ queries. For this reason, the size of the uncertainty region for the $1$-median can become $\Omega(v  n)$. This is true even if we allow the algorithm to query a constant number of objects (instead of one) per unit time. Thus, $O(n)$ is the best possible competitive ratio.
\end{proof}
\end{comment}


The Round-robin algorithm keeps the maximum size of the uncertainty region for the $1$-median within $O(v  n)$. We argue that even for the optimal algorithm, the maximum size of the uncertainty region can be $\Omega(v  n)$.
The proof is presented in Appendix~\ref{app:1m1dOmega}.

\begin{proposition} \label{prop:1m1dOmega}
For the $1$-median problem in $\mathbb{R}^1$, the maximum size of the uncertainty region can be $\Omega(v  n)$ for the optimal algorithm.
\end{proposition}

\begin{comment}
\begin{proof}
We consider an example with $n$ static objects located at the origin. At any point after at least $\lfloor \frac{n}{2} \rfloor$ queries, there will always be at least $\lceil \frac{n}{2} \rceil$ objects that the optimal algorithm will have not acquired their exact locations in the last $\lfloor \frac{n}{2} \rfloor$ queries up to that point. The ending points of the uncertainty regions of those $\lceil \frac{n}{2} \rceil$ objects will be at least $v  \lfloor \frac{n}{2} \rfloor$. Thus, the $(\lfloor \frac{n}{2} \rfloor + 1)$-th smallest ending point among the ending points of the uncertainty regions of all objects will be at least $v  \lfloor \frac{n}{2} \rfloor$. On the other hand, the starting points of the uncertainty regions of all objects will always be less than or equal to zero. Therefore, the size of the uncertainty region for the $(\lfloor \frac{n}{2} \rfloor + 1)$-th smallest problem will be $\Omega(v  n)$ at any point after the first $\lfloor \frac{n}{2} \rfloor$ queries. For this reason, the maximum size of the uncertainty region for the $1$-median problem will be $\Omega(v  n)$ for the optimal algorithm.
\end{proof}
\end{comment}

Next, we provide an upper bound on the competitive ratio of the Round-robin algorithm for the $1$-median problem where objects have different maximum speeds.
The proof is presented in Appendix~\ref{app:1mdiffspeed}.

\begin{proposition} \label{prop:1mdiffspeed}
For the $1$-median problem in $\mathbb{R}^1$ where objects have different maximum speeds, the Round-robin scheduling algorithm achieves a competitive ratio of $O(v_M  n / v_m)$ against the optimal algorithm, where $v_M$ is the highest maximum speed and $v_m$ is the lowest maximum speed.
\end{proposition}

\begin{comment}
\begin{proof}
The Round-robin algorithm keeps the maximum size of the uncertainty region for the $1$-median problem within $O(v_M  n)$. On the other hand, the maximum size of the uncertainty region for the $1$-median problem is $\Omega(v_m)$ for the optimal algorithm. Thus, the competitive ratio of the Round-robin algorithm for the $1$-median problem is $O(v_M  n / v_m)$.
\end{proof}
\end{comment}

Now, we consider the $1$-median problem in $\mathbb{R}^d$ ($d \geq 2$).
The proof of the following proposition is inspired by the proof of Theorem 5.1 of \cite{durocher2006geometric} and can be found in Appendix~\ref{app:1msizeunb}.

\begin{proposition} \label{prop:1msizeunb}
For the $1$-median problem in $\mathbb{R}^d$ ($d \geq 2$), the maximum size of the uncertainty region can be unbounded for the optimal algorithm.
\end{proposition}

\begin{comment}
\begin{proof}
Consider an example with four static objects located at $(0, 0)$, $(0, v)$, $(L, 0)$, and $(L, v)$, where $L$ is arbitrarily large. Regardless of which object is queried first, the uncertainty regions of the objects after the first query suggest that it is possible to have two objects with the exact same location on the line $x = 0$ and two objects with different locations on the line $x = L$. In this case, the $1$-median will be located on the line $x = 0$. Furthermore, the uncertainty regions of the objects after the first query suggest the possibility of having two objects with different locations on the line $x = 0$ and two objects with the exact same location on the line $x = L$. In this case, the $1$-median will be located on the line $x = L$. Therefore, regardless of which object is queried first, the size of the uncertainty region for the $1$-median problem will be at least $L$ which is arbitrarily large. Consequently, the maximum size of the uncertainty region for the $1$-median problem in $d$ dimensions can be unbounded for the optimal algorithm.
\end{proof}
\end{comment}
